Towards Seamless Serverless Computing Across an Edge-Cloud Continuum

Serverless computing has emerged as an attractive paradigm due to the efficiency of development and the ease of deployment without managing any underlying infrastructure. Nevertheless, serverless computing approaches face numerous challenges to unlock their full potential in hybrid environments. To gain a deeper understanding and firsthand knowledge of serverless computing in edge-cloud deployments, we review the current state of open-source serverless platforms and compare them based on predefined requirements. We then design and implement a serverless computing platform with a novel edge orchestration technique that seamlessly deploys serverless functions across the edge and cloud environments on top of the Knative serverless platform. Moreover, we propose an offloading strategy for edge environments and four different functions for experimentation and showcase the performance benefits of our solution. Our results demonstrate that such an approach can efficiently utilize both cloud and edge resources by dynamically offloading functions from the edge to the cloud during high activity, while reducing the overall application latency and increasing request throughput compared to an edge-only deployment.

==> tables/design/github_statistics.tex <==
\begin{sidewaystable}[!htb]
\begin{adjustbox}{width=\textwidth,center=\textwidth}
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l}
\begin{tabular}[c]{@{}l@{}}Serverless\\ platform\end{tabular} & \begin{tabular}[c]{@{}l@{}}GitHub\\ Repositories\end{tabular}                                                                                     & Stars & Forks & \begin{tabular}[c]{@{}l@{}}PRs\\ (active)\end{tabular} & \begin{tabular}[c]{@{}l@{}}PRs\\ (closed)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Issues\\ (open)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Issues\\ (closed)\end{tabular} & Commits & \begin{tabular}[c]{@{}l@{}}Last\\ commit\end{tabular} & Archived \\ \hline \hline
Kyma       & kyma-project/kyma                                                                     & 1368  & 382   & 92            & 9652          & 285            & 4544             & 7499     & 08/06/2022 & No  \\ \hline
Knative             & \begin{tabular}[c]{@{}l@{}}knative/serving\\ knative/eventing\end{tabular} & 5683  & 1400  & 21           & 12881        & 219           & 6246            & 10920   & 07/06/2022 & No  \\ \hline
% KEDA                & kedacore/keda                                                                         & 5048  & 572   & 16           & 1531         & 147           & 1023            & 1465    & 07/06/2022 & No  \\ \hline
OpenFaaS            & openfaas/faas                                                                         & 21656 & 1767  & 3            & 892          & 31            & 753             & 2055    & 06/06/2022 & No  \\ \hline
Fission       & fission/fission                                                                     & 7031  & 706   & 10            & 1425          & 183            & 735             & 1470     & 06/06/2022 & No  \\ \hline
OpenLambda          & open-lambda/open-lambda                                                               & 770   & 86    & 2            & 58           & 9             & 42              & 831     & 02/06/2022 & No  \\ \hline
OpenWhisk           & apache/openwhisk                                                                      & 5700  & 1096  & 39           & 3231         & 319           & 1652            & 2961    & 02/06/2022 & No  \\ \hline
kubeless            & vmware-archive/kubeless                                                               & 6849  & 745   & 3            & 581          & 197           & 471             & 1043    & 15/12/2021 & Yes  \\ \hline
Fn       & fnproject/fn                                                                     & 3010  & 5164   & 382            & 10          & 940            & 135             & 507     & 19/12/2019 & No  \\ \hline
IronFunctions       & iron-io/functions                                                                     & 3010  & 231   & 7            & 386          & 86            & 219             & 904     & 20/08/2018 & No  \\
\end{tabular}
\end{adjustbox}
\caption{Public statistics offered by GitHub for each of the repositories of the open-source serverless platforms as of the $8^{th}$ of June 2022. In cases where there are multiple relevant repositories, we show the cumulative values of all the repositories.}
\label{fig:platform-github-stats}
\end{sidewaystable}

==> tables/design/platform_capabilities.tex <==
\begin{table*}[!ht]
% \begin{adjustbox}{width=1.3\textwidth,center=\textwidth}
\begin{tabular}{ccccccc}
    \toprule
    \textbf{Feature} & 
    % API interface &
    \textbf{Monitoring} &
    \textbf{Orchestrator} &
    \textbf{Cluster support} &
    \textbf{Autoscaling} &
    \textbf{Scale to zero} &
    \begin{tabular}[c]{@{}c@{}}\textbf{Warm instance}\\ \textbf{pool}\end{tabular} \\
    \midrule

    Kyma &
% \begin{tabular}[c]{@{}l@{}}Function (nodejs,\\ python)\end{tabular} &
    \begin{tabular}[c]{@{}c@{}}Prometheus with\\ Grafana\end{tabular} &
    K8S &
    Yes &
    \begin{tabular}[c]{@{}c@{}}Yes (per function;\\ queue-based, cpu-based)\end{tabular} & 

    Yes &
    No \\


    Knative & 
    % Container (http) & 
    \begin{tabular}[c]{@{}c@{}}Prometheus with\\ Grafana\end{tabular} & 
    K8S & 
    Yes & 
    \begin{tabular}[c]{@{}c@{}}Yes (per function;\\ queue-based, cpu-based)\end{tabular} & 
    Yes & 
    No \\


    OpenFaas & 
    % \begin{tabular}[c]{@{}l@{}}Function (nodejs,\\ python, etc)\end{tabular} & 
    \begin{tabular}[c]{@{}c@{}}Prometheus with\\ Grafana\end{tabular} & 
    \begin{tabular}[c]{@{}l@{}}K8S,\\ faasd\end{tabular} & 
    Yes & 
    Yes (global; request rate) & 
    \begin{tabular}[c]{@{}c@{}}No (only available\\ with paid license)\end{tabular} & 
    No  \\
    

    OpenWhisk  & 
    % \begin{tabular}[c]{@{}l@{}}Function (nodejs,\\ python, etc)\end{tabular} & 
    None & 
    K8S & 
    Yes & 
    \begin{tabular}[c]{@{}c@{}}Yes (per function;\\ queue-based)\end{tabular} & 
    Yes & 
    No \\

    Fission    & 
    % \begin{tabular}[c]{@{}l@{}}Function (nodejs,\\ python, etc)\end{tabular} & 
    \begin{tabular}[c]{@{}c@{}}Prometheus with\\ Grafana\end{tabular} & 
    K8S & 
    Yes & 
    Yes (per function) & 
    Yes & 
    Yes \\

    OpenLambda & 
    % Function (python) & 
    None & 
    - & 
    No & 
    Yes (per function) & 
    Yes & 
    No \\
    \bottomrule
\end{tabular}
% \end{adjustbox}
\caption{Platform capabilities relevant to the defined requirements.}
\label{fig:platform-capabilities}
\end{table*}

==> tables/setup/constants.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        \textbf{Constant} & \textbf{Value} & \textbf{Source} \\
        \hline
        $c_{soft}$ & $1.25$ & Equation \eqref{eq:r-traffic} \\
        \hline
        $c_{hard}$ & $2.0$ & Equation \eqref{eq:r-traffic} \\
        \hline
        $c_{inertia}$ & $0.6667$ & Equation \eqref{eq:prometheus-final-traffic} \\
        \hline
        $c_{decay}$ & $0.5$ & Equation \eqref{eq:rp-traffic} \\
        \hline
    \end{tabular}
    \caption{In the implementation of the offloading strategy, a set of values for the constants were selected based on what was deemed to be sensible. While it is feasible to set the constants individually for each function in Knative Edge, it was determined that the chosen values were sufficient for the needs of the implementation without undergoing further optimization specifically for the use case.}
    \label{tab:experiment-3-scheduler-constants}
\end{table}

==> tables/setup/specs.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        \textbf{Type} & \textbf{CPU} & \textbf{Memory} & \textbf{Storage} \\
        \hline
        Cloud Virtual Machine & 4 vCPUs & 16GB & 160GB NVMe \\
        \hline
        Edge device & 2 x64 cores @ 1.6GHz & 4GB & 64GB Flash \\
        \hline
        Raspberry Pi 3 B+ & 4 ARMv8 cores @ 1.4GHz & 1GB & 32GB Flash \\
        \hline
    \end{tabular}
    \caption{The experiment includes several devices, each with specific hardware specifications. The edge cluster is comprised of an edge device and four Raspberry Pis, while the cloud cluster consists of a single virtual machine (VM).}
    \label{tab:all-configs-specs}
\end{table}

==> tables/setup/versions.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \textbf{Type} & \textbf{OS} & \textbf{Kubernetes} & \textbf{Knative} \\
        \hline
        Low-powered PC & Alpine Linux v3.15.6 & 1.24.3 & 1.7 \\
        \hline
        Raspberry Pi 3 B+ & Alpine Linux v3.15.6 & 1.24.3 & 1.7 \\
        \hline
        Virtual machine & Ubuntu 22.04.1 LTS & 1.24.3 & 1.7 \\
        \hline
    \end{tabular}
    \caption{The software versions utilized in the experiments were kept consistent across all devices. The edge devices were equipped with a lightweight Linux distribution, Alpine Linux, while the cloud virtual machine was utilizing an Ubuntu image. The version compatibility of both Kubernetes and Knative was maintained uniformly across the cloud and edge devices.}
    \label{tab:all-configs-versions}
\end{table}

==> tables/setup/workloads.tex <==
\begin{table}[!thb]
    \centering
    \caption{For each category of experiment workload, we provide an expected impact analysis on the usage of CPU, memory, disk, and network resources.}
    \label{tab:experiment-3-fn-categories}
    \begin{tabular}{ccccc}
        \toprule
        \textbf{Workload} & \textbf{CPU} & \textbf{Memory} & \textbf{Disk} & \textbf{Network} \\
        \midrule
        Matrix Multiplication & high & medium & none & medium \\
        Image Processing & medium & medium & low & low \\
        Random I/O & low & low & high & none \\
        Mixed & high & medium & high & medium \\
        \bottomrule
    \end{tabular}
    % \caption{For each category of experiment workload, we list the expected impact on the CPU, memory, disk, and network usage. For the last workload, we combine all three workloads at the same time.}
    
\end{table}

==> tables/setup/workloads_description.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        \textbf{Option} & \textbf{Value} & \textbf{Note} \\
        \hline
        \makecell{Experiment \\concurrency limit} & $8$ & \makecell{A limit was set in order to allows Knative to scale the \\functions before overloading a single edge node.} \\
        \hline
        \makecell{Experiment \\concurrency target} & $4$ & \makecell{The intended level of concurrency was established at \\half the maximum concurrency limit to facilitate the \\scaling down of the function.} \\
        \hline
        \makecell{Experiment \\max scale} & $8$ & \makecell{If not set, Knative will scale function instances based on the \\concurrency target, even if nodes are being overloaded. \\To prevent cluster failures, it is necessary to set a limit.} \\
        \hline
        \makecell{Edge proxy \\min scale} & $3$ & \makecell{A lower limit was set over 0 to ensure consistent experiment \\results, as allowing the Edge proxy to scale to zero leads \\to inconsistent results.} \\
        \hline
        \makecell{Edge proxy \\max scale} & $5$ & \makecell{A limit was set to prevent the creation of excessive Edge proxy \\instances, as the container is I/O bound and having more \\instances than worker nodes can be inefficient.} \\
        \hline
    \end{tabular}
    \caption{In order to optimize the functions for execution on edge devices and to achieve consistent experimental results, modifications were made to the default run-time options provided by Knative.}
    \label{tab:experiment-3-knative-config}
\end{table}

==> tables/setup/workloads_requests.tex <==
\begin{table}[!thb]
    \centering
    \begin{tabular}{cccc}
        \toprule
        \textbf{Workload} & \textbf{Min load} & \textbf{Max load} & \textbf{Total} \\
        \midrule
        Matrix multiplication & 1 req/s & 5 req/s & 2700 \\
        Image processing & 1 req/s & 8 req/s & 4050 \\
        Random I/O & 1 req/s & 20 req/s & 9450 \\
        Mixed & 1+1+1 req/s & 4+8+8 req/s & 10350 \\
        \bottomrule
    \end{tabular}
    \caption{For the first 5 minutes of an experiment run, we make requests at the minimum load. Afterwards, we linearly increase the number of requests made until we read the maximum load at 10 minutes. Finally, we continue making requests at that rate for another 5 minutes. For the mixed workload, we show the minimum and maximum load as the sum of the previous workloads, in the order they are in the rows above.}
    \label{tab:experiment-3-load}
\end{table}
